Interplay between core and corona components in high-energy nuclear collisions

We establish the updated version of dynamical core--corona initialization framework (DCCI2) as a unified description from small to large colliding systems and from low to high transverse momentum ($p_T$) regions. Using DCCI2, we investigate effects of interplay between locally equilibrated and non-equilibrated systems, in other words, core and corona components in high-energy nuclear collisions. Given experimental multiplicity distributions and yield ratios of $\Omega$ baryons to charged pions as inputs, we extract the fraction of core and corona components in p+p collisions at $\sqrt{s}=7$ TeV and Pb+Pb collisions at $\sqrt{s_{NN}}=2.76$ TeV. We find core contribution overtakes corona contribution as increasing multiplicity above $\langle dN_{\mathrm{ch}}/d\eta \rangle_{|\eta|<0.5} \sim 18$ regardless of the collision system or energy. We also see that the core contribution exceeds the corona contribution only in 0.0-0.95\% multiplicity class in p+p collisions. Notably, there is a small enhancement of corona contribution with $\sim20$\% below $p_T\sim 1$ GeV even in minimum bias Pb+Pb collisions. We find that the corona contribution at low $p_T$ gives $\sim 15$-$38$ $\%$ correction on $v_2\{2\}$ at $N_{\mathrm{ch}}\lesssim 370$. This raises a problem in conventional hydrodynamic analyses in which low $p_T$ soft hadrons originate solely from core components. We finally scrutinize the roles of string fragmentation and the longitudinal expansion in the transverse energy per unit rapidity, which is crucial in initial conditions for hydrodynamics from event generators based on string models.

==> Introduction.tex <==
Quark-gluon plasma (QGP) is a state of thermalized and chemically equilibrated matter consisting of quarks and gluons deconfined from hadrons at extremely high temperature and density.
High-energy nuclear collision experiments in the Relativistic Heavy Ion Collider (RHIC) at Brookhaven National Laboratory 
and at the Large Hadron Collider (LHC) in CERN
provide opportunities to explore properties of the extreme state.

Relativistic hydrodynamics is proven to successfully describe experimental data of relativistic heavy-ion collisions since the first discovery of hydrodynamic behavior of the QGP in the early 2000s \cite{Heinz:2001xi,Gyulassy:2004zy,Shuryak:2004cy,Hirano:2005wx}.
Since final observables reflect all the history of the reaction, it is of significant importance to model each stage of the reaction and to integrate these modules as a whole in a consistent way towards a further comprehensive understanding of the QGP \cite{Hirano:2012kj}. In particular, modeling of initial pre-equilibrium and final decoupling stages is needed in addition to a relativistic hydrodynamic model as a framework to describe transient states. 
Notably, there are some attempts to constrain transport coefficients of the QGP by using state-of-the-art dynamical models based on relativistic hydrodynamics \cite{Bernhard:2019bmu,Nijs:2020ors,Everett:2020xug}.
As one sees from this, the QGP study is in the middle of a transition to precision science. 

Despite the great success of dynamical models based on relativistic hydrodynamics in describing a vast body of experimental data, it poses some open issues for a comprehensive description of the whole reaction in high-energy nuclear collisions.
One of the major issues is an initial condition of relativistic hydrodynamic equations which does not respect the total energy of the colliding systems.
Initial conditions have been parametrized and put to reproduce centrality dependence of multiplicity or pseudorapidity distributions in a conventional hydrodynamic approach.
As a result, the total energy of the initial hydrodynamic fields does not exactly match the collision energy of the system. 
Even when some outputs from event generators with a given collision system and energy are utilized for initial conditions in hydrodynamic models, an additional scale parameter is commonly introduced to adjust the model outputs of multiplicity. 
%Reference for AMPT initial conditions. How about IP-Glasma case???
One might not think it is necessary for the energy of the initial hydrodynamic fields to be the same as the total energy of the system.
This is exactly a starting point of our discussion in a series of papers \cite{Okai:2017ofp,Kanakubo:2018vkl,Kanakubo:2019ogh}: The relativistic hydrodynamics merely describes a part of system, namely, matter in local equilibrium, while other parts of the system such as propagating jets and matter out of equilibrium are to be described at the same time.

First attempts of simultaneous description of both the QGP fluids in equilibrium and the energetic partons out of equilibrium had been made in Refs.~\cite{Hirano:2002sc,Hirano:2003hq,Hirano:2003yp,Hirano:2003pw,Hirano:2004en} \footnote{Note that the very first study to utilize the hydrodynamic solutions in quantitative analysis of parton energy loss was done in Ref.~\cite{Gyulassy:2001kr}.}.
Initial conditions in those studies were still either parametrized via an optical Glauber model \cite{Glauber:2006gd} or taken from a saturation model \cite{Kharzeev:2000ph,Kharzeev:2001gp,Kharzeev:2001yq,Kharzeev:2002ei} so as to reproduce yields of low $p_T$ hadrons, while hard partons which undergo energy loss during traversing QGP fluids were supplemented to successfully reproduce the hadron spectra from low to high $p_{T}$ regions \cite{Hirano:2002sc,Hirano:2003yp,Hirano:2004en}.
It was found that an intriguing interplay between soft and hard components brought ones to interpretation of the proton yield anomaly in $p_{T}$ spectra \cite{Hirano:2003yp}.
However, the model lacked back reactions from quenching partons to the QGP fluids and a contribution from fragmentation was cut in low $p_T$ regions, both of which obviously violate the energy-momentum conservation law.

%Hydro + source terms
Medium responses to propagating energetic partons have been modeled within hydrodynamic equations with source terms by assuming the instantaneous equilibration of the deposited energy and momentum from partons \cite{Stoecker:2004qu,CasalderreySolana:2004qm,Satarov:2005mv,Renk:2005si,Chaudhuri:2005vc,Chaudhuri:2006qk,Chaudhuri:2007vc,Betz:2010qh,Tachibana:2014lja,Tachibana:2015qxa,Tachibana:2017syd,Chen:2017zte,Chang:2019sae,Tachibana:2020mtb,Zhao:2021vmu}.
Within this approach, the sum of the energy and momentum of fluids and those of traversing partons is conserved as a whole. However, it is not clear how to divide the initial system just after the collision into soft (fluids in equilibrium) and hard (partons out of equilibrium) parts.

%Dynamical initialization
To remedy this issue, a dynamical initialization model \cite{Okai:2017ofp} was proposed to describe the dynamics of gradually forming QGP fluids phenomenologically \footnote{Dynamical initialization is essential in describing the formation of fluids in lower collision energies in which secondary hadrons are gradually produced in finite time duration due to insufficient Lorentz contraction of colliding nuclei \cite{Shen:2017bsr,Akamatsu:2018olk}.
}.
In contrast to the conventional hydrodynamic models in which initial conditions are put at a fixed initial time, the QGP fluids are generated locally in time and space in the dynamical initialization framework.
Under this framework, all the input of energy-momentum of QGP fluids is the one of partons produced just after the nuclear collisions. 
Starting with vacuum, energy-momentum of the QGP fluids is dynamically generated by solving hydrodynamic equations with source terms. 
% \sout{, where the source term is defined as a phenomenological fluidization rate, \textit{i.e.}, the four-momentum deposition per unit time for a parton}
Consequently, fluids in local equilibrium are generated from the initial partons by depositing the energy and the momentum and surviving partons are considered to remain out of equilibrium.
When initial partons are taken, \textit{e.g.}, from event generators, the total energy keeps its value of the colliding two nuclei all the way through the dynamical initialization. 
Although we successfully separated matter in local equilibrium from initially produced partons in the dynamical initialization framework \cite{Okai:2017ofp}, the fluidization scheme was too simple and phenomenological to describe the transverse momentum spectra and the particle ratios.
Then, we introduced the core--corona picture into the dynamical initialization.


%Explain differences from EPOS
%--------------------------------
The conventional core--corona picture was proposed to explain centrality dependence of strange hadron yield ratios~\cite{Werner:2007bf}. 
As multiplicity increases, the high-density region, in which the matter is mostly thermalized, is supposed to become larger. 
As a result, the final hadron yields become dominated by the hadrons from thermalized matter rather than non-thermalized matter created in low-density regions. 
The former component is referred to as core, while the latter one is referred to as corona. 

A Monte-Carlo event generator, EPOS~\cite{Pierog:2013ria,Werner:2018yad} is widely accepted for its implementation of the core--corona picture. In the latest study in Refs.~\cite{Werner:2013tya,Werner:2019aqa}, string segments produced in a collision are separated sharply into the core and the corona components depending on their density and transverse momentum at a fixed time. Low-$p_T$ string segments in dense regions are fully converted into the thermalized medium fluid, while string segments with high momentum or dilute regions are directly hadronized.

On the other hand, we model the dynamical aspects of the core--corona separation introducing the particle density dependence of the dynamical initialization scheme, which is called the \textit{dynamical core--corona initialization (DCCI)}  \cite{Kanakubo:2018vkl,Kanakubo:2019ogh} \footnote{In fact, this idea was first implemented in Ref.~\cite{Akamatsu:2018olk} to describe excitation functions of particle ratios at lower collision energies. However, it was applied to the secondary produced hadrons rather than partons.}.
One of the key features of the DCCI is to deal with dynamics of the core (equilibrium) and the corona (non-equilibrium) at the same time.
With the description of the dynamics, gradual formation of core and corona in spatial and momentum space is achieved.
In the DCCI framework, the multiplicity dependence of the hadron yield ratios of multi-strange baryons to pions from small to large colliding systems in a wide range of collision energy is attributed to a continuous change of the fractions of the core and the corona components as multiplicity increases \cite{Kanakubo:2018vkl,Kanakubo:2019ogh}.
It should be noted here that the ``corona" is referred not only to an outer layer in the coordinate space but also to the one in the momentum space:
The lower $p_T$ partons are more likely to deposit their energy and momentum to form the fluids and the higher $p_T$ partons are less likely to be equilibrated during the DCCI processes.

%Summary of new features in DCCI2
%-------------------------------
In this paper, we update the DCCI framework towards a more comprehensive description of dynamics in full phase space from small to large colliding systems in a unified manner.
Hereafter we call this updated DCCI the \textit{DCCI2}.
In comparison with the previous work \cite{Kanakubo:2018vkl,Kanakubo:2019ogh}, several crucial updates have been made in this new version including a more sophisticated formula for four-momentum deposition of initial partons, particlization of the fluids on the switching hypersurface through a Monte-Carlo sampler \ISthreeD\  \cite{McNelis:2019auj}, hadronic rescatterings through a hadron cascade model \jam\  \cite{Nara:1999dz}, and modification of structure of color strings inside the fluids.
With these updates, the DCCI2 is capable of describing high-energy nuclear collisions from low to high $p_T$ region with particle identification in various colliding systems.

We generate initial partons from a general-purpose event generator \pythia8 \cite{Sjostrand:2007gs, Bierlich:2014xba}
switching off hadronization and make all of them sources of both the core and the corona parts. 
Here a special emphasis is put on to discriminate between the two terms, ``soft--hard" and ``core--corona". We call the core when it composes the matter in equilibrium. 
In DCCI2, the fluids generated through the dynamical initialization correspond to the core part and hardons particlized on switching hypersurface are regarded as the core components.
On the other hand, we call the corona when it composes matter completely out of equilibrium. 
In DCCI2, partons in the dilute regions and/or surviving even through the dynamical initialization correspond to the corona part, and hadrons from string decays are regarded as the corona components.
Although the core (corona) component is sometimes identified with the soft (hard) component, it is not the case in the DCCI2: The hadrons from string fragmentation are distributed all the way down to very low $p_T$ region, which one cannot consider as ``hard" components.
To the best of our knowledge, it has been believed so far without any strong justification that the corona components would be negligible in low $p_T$ region in heavy-ion collisions.
In this paper, we scrutinize 
the size of the contribution from the corona components 
in soft observables (``soft-from-corona") 
and how the fraction of the corona components evolves as multiplicity increases.

One of the main interests in this field is to constrain the transport coefficients of the QGP through the hydrodynamic analysis of anisotropic flow data in low $p_T$ regions.
It is conventionally assumed that the low $p_T$ hadrons are completely dominated by the core components. 
What if the corona components, whose contribution is often considered to be very small, affect the bulk observables in heavy-ion collisions?  
The non-equilibrium contribution is at most taken through small corrections to thermodynamic quantities such as shear stress and bulk pressure. 
Since the corona components are far-from-equilibrium distributions, these must be more important than those dissipative corrections in the hydrodynamic analysis if these are smaller than the core components, but of the same order of the magnitude.
Thus, dynamical modeling containing the core--corona picture could become the next-generation model inevitably needed for the precision study of the QGP properties. 

The present paper is organized as follow:
We explain details about the DCCI2 model in Sec.~\ref{sec:model}.
Staring from the general idea of dynamical initialization and the dynamical core--corona initialization,
we discuss some new features in the DCCI2 model.
In Sec.~\ref{sec:results}, we show the results from the DCCI2 model in p+p and Pb+Pb collisions at the LHC energies.
We also discuss the effects of string fragmentation and the longitudinal hydrodynamic expansion on the transverse energy per unit rapidity which play a crucial role in modeling hydrodynamic initial conditions. 
Section \ref{sec:summary} is devoted to the summary of the present paper.

Throughout this paper, 
we use the natural unit, $\hbar = c = k_{B} =1$, and the Minkowski metric,
$g_{\mu \nu} = \mathrm{diag}(1, -1, -1, -1)$.


